Comprehensive analysis of local and nonlocal amplitudes in the $B^0\rightarrow K^{*0}\mu^+\mu^-$ decay

A comprehensive study of the local and nonlocal amplitudes contributing to the decay $B^0\rightarrow K^{*0}(\to K^+\pi^-) \mu^+\mu^-$ is performed by analysing the phase-space distribution of the decay products. The analysis is based on $pp$ collision data corresponding to an integrated luminosity of 8.4fb$^{-1}$ collected by the LHCb experiment. This measurement employs for the first time a model of both one-particle and two-particle nonlocal amplitudes, and utilises the complete dimuon mass spectrum without any veto regions around the narrow charmonium resonances. In this way it is possible to explicitly isolate the local and nonlocal contributions and capture the interference between them. The results show that interference with nonlocal contributions, although larger than predicted, only has a minor impact on the Wilson Coefficients determined from the fit to the data. For the local contributions, the Wilson Coefficient $C_9$, responsible for vector dimuon currents, exhibits a $2.1\sigma$ deviation from the Standard Model expectation. The Wilson Coefficients $C_{10}$, $C_{9}'$ and $C_{10}'$ are all in better agreement than $C_{9}$ with the Standard Model and the global significance is at the level of $1.5\sigma$. The model used also accounts for nonlocal contributions from $B^{0}\to K^{*0}\left[\tau^+\tau^-\to \mu^+\mu^-\right]$ rescattering, resulting in the first direct measurement of the $b s\tau\tau$ vector effective-coupling $C_{9\tau}$.

==> Authorship_LHCb-PAPER-2024-011-arXiv.tex <==
LHCb collaboration:
R. Aaij,
A.S.W. Abdelmotteleb,
C. Abellan Beteta,
F. Abudin{\'e}n,
T. Ackernley,
A. A.  Adefisoye,
B. Adeva,
M. Adinolfi,
P. Adlarson,
C. Agapopoulou,
C.A. Aidala,
Z. Ajaltouni,
S. Akar,
K. Akiba,
P. Albicocco,
J. Albrecht,
F. Alessio,
M. Alexander,
Z. Aliouche,
P. Alvarez Cartelle,
R. Amalric,
S. Amato,
J.L. Amey,
Y. Amhis,
L. An,
L. Anderlini,
M. Andersson,
A. Andreianov,
P. Andreola,
M. Andreotti,
D. Andreou,
A. Anelli,
D. Ao,
F. Archilli,
M. Argenton,
S. Arguedas Cuendis,
A. Artamonov,
M. Artuso,
E. Aslanides,
R. Ataide Da Silva,
M. Atzeni,
B. Audurier,
D. Bacher,
I. Bachiller Perea,
S. Bachmann,
M. Bachmayer,
J.J. Back,
P. Baladron Rodriguez,
V. Balagura,
W. Baldini,
H.  Bao,
J. Baptista de Souza Leite,
M. Barbetti,
I. R. Barbosa,
R.J. Barlow,
M. Barnyakov,
S. Barsuk,
W. Barter,
M. Bartolini,
J. Bartz,
J.M. Basels,
G. Bassi,
B. Batsukh,
A. Bay,
A. Beck,
M. Becker,
F. Bedeschi,
I.B. Bediaga,
S. Belin,
V. Bellee,
K. Belous,
I. Belov,
I. Belyaev,
G. Benane,
G. Bencivenni,
E. Ben-Haim,
A. Berezhnoy,
R. Bernet,
S. Bernet Andres,
A. Bertolin,
C. Betancourt,
F. Betti,
J.  Bex,
Ia. Bezshyiko,
J. Bhom,
M.S. Bieker,
N.V. Biesuz,
P. Billoir,
A. Biolchini,
M. Birch,
F.C.R. Bishop,
A. Bitadze,
A. Bizzeti,
T. Blake,
F. Blanc,
J.E. Blank,
S. Blusk,
V. Bocharnikov,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A.  Bohare,
A. Boldyrev,
C.S. Bolognani,
R. Bolzonella,
N. Bondar,
F. Borgato,
S. Borghi,
M. Borsato,
J.T. Borsuk,
S.A. Bouchiba,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
A. Brea Rodriguez,
N. Breer,
J. Brodzicka,
A. Brossa Gonzalo,
J. Brown,
D. Brundu,
E. Buchanan,
A. Buonaura,
L. Buonincontri,
A.T. Burke,
C. Burr,
A. Butkevich,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
R. Calabrese,
S. Calderon Ramirez,
L. Calefice,
S. Cali,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
J. I. Cambon Bouzas,
P. Campana,
D.H. Campora Perez,
A.F. Campoverde Quezada,
S. Capelli,
L. Capriotti,
R. Caravaca-Mora,
A. Carbone,
L. Carcedo Salgado,
R. Cardinale,
A. Cardini,
P. Carniti,
L. Carus,
A. Casais Vidal,
R. Caspary,
G. Casse,
J. Castro Godinez,
M. Cattaneo,
G. Cavallero,
V. Cavallini,
S. Celani,
D. Cervenkov,
S.  Cesare,
A.J. Chadwick,
I. Chahrour,
M. Charles,
Ph. Charpentier,
E.  Chatzianagnostou,
C.A. Chavez Barajas,
M. Chefdeville,
C. Chen,
S. Chen,
Z. Chen,
A. Chernov,
S. Chernyshenko,
V. Chobanova,
S. Cholak,
M. Chrzaszcz,
A. Chubykin,
V. Chulikov,
P. Ciambrone,
X. Cid Vidal,
G. Ciezarek,
P. Cifra,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
C. Cocha Toapaxi,
V. Coco,
J. Cogan,
E. Cogneras,
L. Cojocariu,
P. Collins,
T. Colombo,
A. Comerma-Montells,
L. Congedo,
A. Contu,
N. Cooke,
I. Corredoira ,
A. Correia,
G. Corti,
J.J. Cottee Meldrum,
B. Couturier,
D.C. Craik,
M. Cruz Torres,
E. Curras Rivera,
R. Currie,
C.L. Da Silva,
S. Dadabaev,
L. Dai,
X. Dai,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
J. Daniel,
A. Danilina,
P. d'Argent,
A.  Davidson,
J.E. Davies,
A. Davis,
O. De Aguiar Francisco,
C. De Angelis,
F. De Benedetti,
J. de Boer,
K. De Bruyn,
S. De Capua,
M. De Cian,
U. De Freitas Carneiro Da Graca,
E. De Lucia,
J.M. De Miranda,
L. De Paula,
M. De Serio,
P. De Simone,
F. De Vellis,
J.A. de Vries,
F. Debernardis,
D. Decamp,
V. Dedu,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
J. Deng,
V. Denysenko,
O. Deschamps,
F. Dettori,
B. Dey,
P. Di Nezza,
I. Diachkov,
S. Didenko,
S. Ding,
L. Dittmann,
V. Dobishuk,
A. D.  Docheva,
C. Dong,
A.M. Donohoe,
F. Dordei,
A.C. dos Reis,
A. D.  Dowling,
W. Duan,
P. Duda,
M.W. Dudek,
L. Dufour,
V. Duk,
P. Durante,
M. M. Duras,
J.M. Durham,
O. D.  Durmus,
A. Dziurda,
A. Dzyuba,
S. Easo,
E. Eckstein,
U. Egede,
A. Egorychev,
V. Egorychev,
S. Eisenhardt,
E. Ejopu,
L. Eklund,
M. Elashri,
J. Ellbracht,
S. Ely,
A. Ene,
E. Epple,
J. Eschle,
S. Esen,
T. Evans,
F. Fabiano,
L.N. Falcao,
Y. Fan,
B. Fang,
L. Fantini,
M. Faria,
K.   Farmer,
D. Fazzini,
L. Felkowski,
M. Feng,
M. Feo,
M. Fernandez Gomez,
A.D. Fernez,
F. Ferrari,
F. Ferreira Rodrigues,
M. Ferrillo,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
K.M. Fischer,
D.S. Fitzgerald,
C. Fitzpatrick,
F. Fleuret,
M. Fontana,
L. F.  Foreman,
R. Forty,
D. Foulds-Holt,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Q. Fuehring,
Y. Fujii,
T. Fulghesu,
E. Gabriel,
G. Galati,
M.D. Galati,
A. Gallas Torreira,
D. Galli,
S. Gambetta,
M. Gandelman,
P. Gandini,
B.  Ganie,
H. Gao,
R. Gao,
Y. Gao,
Y. Gao,
Y. Gao,
M. Garau,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc{\'\i}a Pardi{\~n}as,
K. G.  Garg,
L. Garrido,
C. Gaspar,
R.E. Geertsema,
L.L. Gerken,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
Z. Ghorbanimoghaddam,
L. Giambastiani,
F. I. Giasemis,
V. Gibson,
H.K. Giemza,
A.L. Gilman,
M. Giovannetti,
A. Giovent{\`u},
P. Gironella Gironell,
C. Giugliano,
M.A. Giza,
E.L. Gkougkousis,
F.C. Glaser,
V.V. Gligorov,
C. G{\"o}bel,
E. Golobardes,
D. Golubkov,
A. Golutvin,
A. Gomes,
S. Gomez Fernandez,
F. Goncalves Abrantes,
M. Goncerz,
G. Gong,
J. A. Gooding,
I.V. Gorelov,
C. Gotti,
J.P. Grabowski,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
L. Grazette,
G. Graziani,
A. T. Grecu,
L.M. Greeven,
N.A. Grieser,
L. Grillo,
S. Gromov,
C.  Gu,
M. Guarise,
M. Guittiere,
V. Guliaeva,
P. A. G{\"u}nther,
A.-K. Guseinov,
E. Gushchin,
Y. Guz,
T. Gys,
K. Habermann,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
J. Haimberger,
M. Hajheidari,
M.M. Halvorsen,
P.M. Hamilton,
J. Hammerich,
Q. Han,
X. Han,
S. Hansmann-Menzemer,
L. Hao,
N. Harnew,
M. Hartmann,
J. He,
M. Hecker,
F. Hemmer,
C. Henderson,
R.D.L. Henderson,
A.M. Hennequin,
K. Hennessy,
L. Henry,
J. Herd,
P. Herrero Gascon,
J. Heuel,
A. Hicheur,
G. Hijano Mendizabal,
D. Hill,
S.E. Hollitt,
J. Horswill,
R. Hou,
Y. Hou,
N. Howarth,
J. Hu,
J. Hu,
W. Hu,
X. Hu,
W. Huang,
W. Hulsbergen,
R.J. Hunter,
M. Hushchyn,
D. Hutchcroft,
D. Ilin,
P. Ilten,
A. Inglessi,
A. Iniukhin,
A. Ishteev,
K. Ivshin,
R. Jacobsson,
H. Jage,
S.J. Jaimes Elles,
S. Jakobsen,
E. Jans,
B.K. Jashal,
A. Jawahery,
V. Jevtic,
E. Jiang,
X. Jiang,
Y. Jiang,
Y. J.  Jiang,
M. John,
D. Johnson,
C.R. Jones,
T.P. Jones,
S. Joshi,
B. Jost,
N. Jurik,
I. Juszczak,
D. Kaminaris,
S. Kandybei,
M.  Kane,
Y. Kang,
C. Kar,
M. Karacson,
D. Karpenkov,
A. Kauniskangas,
J.W. Kautz,
F. Keizer,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
S. Kholodenko,
G. Khreich,
T. Kirn,
V.S. Kirsebom,
O. Kitouni,
S. Klaver,
N. Kleijne,
K. Klimaszewski,
M.R. Kmiec,
S. Koliiev,
L. Kolk,
A. Konoplyannikov,
P. Kopciewicz,
P. Koppenburg,
M. Korolev,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
A. Kozachuk,
P. Kravchenko,
L. Kravchuk,
M. Kreps,
P. Krokovny,
W. Krupa,
W. Krzemien,
O.K. Kshyvanskyi,
J. Kubat,
S. Kubis,
M. Kucharczyk,
V. Kudryavtsev,
E. Kulikova,
A. Kupsc,
B. K.  Kutsenko,
D. Lacarrere,
A. Lai,
A. Lampis,
D. Lancierini,
C. Landesa Gomez,
J.J. Lane,
R. Lane,
C. Langenbruch,
J. Langer,
O. Lantwin,
T. Latham,
F. Lazzari,
C. Lazzeroni,
R. Le Gac,
R. Lef{\`e}vre,
A. Leflat,
S. Legotin,
M. Lehuraux,
E. Lemos Cid,
O. Leroy,
T. Lesiak,
B. Leverington,
A. Li,
H. Li,
K. Li,
L. Li,
P. Li,
P.-R. Li,
Q.  Li,
S. Li,
T. Li,
T. Li,
Y. Li,
Y. Li,
Z. Lian,
X. Liang,
S. Libralon,
C. Lin,
T. Lin,
R. Lindner,
V. Lisovskyi,
R. Litvinov,
F. L.  Liu,
G. Liu,
K. Liu,
S. Liu,
Y. Liu,
Y. Liu,
Y. L.  Liu,
A. Lobo Salvia,
A. Loi,
J. Lomba Castro,
T. Long,
J.H. Lopes,
A. Lopez Huertas,
S. L{\'o}pez Soli{\~n}o,
C. Lucarelli,
D. Lucchesi,
M. Lucio Martinez,
V. Lukashenko,
Y. Luo,
A. Lupato,
E. Luppi,
K. Lynch,
X.-R. Lyu,
G. M.  Ma,
R. Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
B.  Mack,
I. Mackay,
L. M.  Mackey,
L.R. Madhan Mohan,
M. M.  Madurai,
A. Maevskiy,
D. Magdalinski,
D. Maisuzenko,
M.W. Majewski,
J.J. Malczewski,
S. Malde,
L. Malentacca,
A. Malinin,
T. Maltsev,
G. Manca,
G. Mancinelli,
C. Mancuso,
R. Manera Escalero,
D. Manuzzi,
D. Marangotto,
J.F. Marchand,
R. Marchevski,
U. Marconi,
S. Mariani,
C. Marin Benito,
J. Marks,
A.M. Marshall,
G. Martelli,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
A. Massafferri,
R. Matev,
A. Mathad,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
J. Mauricio,
P. Mayencourt,
M. Mazurek,
M. McCann,
L. Mcconnell,
T.H. McGrath,
N.T. McHugh,
A. McNab,
R. McNulty,
B. Meadows,
G. Meier,
D. Melnychuk,
F. M.  Meng,
M. Merk,
A. Merli,
L. Meyer Garcia,
D. Miao,
H. Miao,
M. Mikhasenko,
D.A. Milanes,
A. Minotti,
E. Minucci,
T. Miralles,
B. Mitreska,
D.S. Mitzel,
A. Modak,
A. M{\"o}dden ,
R.A. Mohammed,
R.D. Moise,
S. Mokhnenko,
T. Momb{\"a}cher,
M. Monk,
S. Monteil,
A. Morcillo Gomez,
G. Morello,
M.J. Morello,
M.P. Morgenthaler,
A.B. Morris,
A.G. Morris,
R. Mountain,
H. Mu,
Z. M.  Mu,
E. Muhammad,
F. Muheim,
M. Mulder,
K. M{\"u}ller,
F. Mu{\~n}oz-Rojas,
R. Murta,
P. Naik,
T. Nakada,
R. Nandakumar,
T. Nanut,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
P. Neustroev,
J. Nicolini,
D. Nicotra,
E.M. Niel,
N. Nikitin,
P. Nogarolli,
P. Nogga,
N.S. Nolte,
C. Normand,
J. Novoa Fernandez,
G. Nowak,
C. Nunez,
H. N.  Nur,
A. Oblakowska-Mucha,
V. Obraztsov,
T. Oeser,
S. Okamura,
A. Okhotnikov,
O. Okhrimenko,
R. Oldeman,
F. Oliva,
M. Olocco,
C.J.G. Onderwater,
R.H. O'Neil,
J.M. Otalora Goicochea,
P. Owen,
A. Oyanguren,
O. Ozcelik,
A.  Padee,
K.O. Padeken,
B. Pagare,
P.R. Pais,
T. Pajero,
A. Palano,
M. Palutan,
G. Panshin,
L. Paolucci,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
C. Parkes,
B. Passalacqua,
G. Passaleva,
D. Passaro,
A. Pastore,
M. Patel,
J. Patoc,
C. Patrignani,
A.  Paul,
C.J. Pawley,
A. Pellegrino,
J.  Peng,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
H.  Pereira Da Costa,
A. Pereiro Castro,
P. Perret,
A. Perro,
K. Petridis,
A. Petrolini,
J. P.  Pfaller,
H. Pham,
L. Pica,
M. Piccini,
B. Pietrzyk,
G. Pietrzyk,
D. Pinci,
F. Pisani,
M. Pizzichemi,
V. Placinta,
M. Plo Casasus,
F. Polci,
M. Poli Lener,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
G.J. Pomery,
S. Ponce,
D. Popov,
S. Poslavskii,
K. Prasanth,
C. Prouve,
V. Pugatch,
G. Punzi,
S.  Qasim,
Q. Q.  Qian,
W. Qian,
N. Qin,
S. Qu,
R. Quagliani,
R.I. Rabadan Trejo,
J.H. Rademacker,
M. Rama,
M.  Ram\'{i}rez Garc\'{i}a,
V. Ramos De Oliveira,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Rebollo De Miguel,
F. Redi,
J. Reich,
F. Reiss,
Z. Ren,
P.K. Resmi,
R. Ribatti,
G. R.  Ricart,
D. Riccardi,
S. Ricciardi,
K. Richardson,
M. Richardson-Slipper,
K. Rinnert,
P. Robbe,
G. Robertson,
E. Rodrigues,
E. Rodriguez Fernandez,
J.A. Rodriguez Lopez,
E. Rodriguez Rodriguez,
A. Rogovskiy,
D.L. Rolf,
P. Roloff,
V. Romanovskiy,
M. Romero Lamas,
A. Romero Vidal,
G. Romolini,
F. Ronchetti,
T. Rong,
M. Rotondo,
S. R.  Roy,
M.S. Rudolph,
T. Ruf,
M. Ruiz Diaz,
R.A. Ruiz Fernandez,
J. Ruiz Vidal,
A. Ryzhikov,
J. Ryzka,
J. J. Saavedra-Arias,
J.J. Saborido Silva,
R. Sadek,
N. Sagidova,
D. Sahoo,
N. Sahoo,
B. Saitta,
M. Salomoni,
C. Sanchez Gras,
I. Sanderswood,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
L. Santoro ,
E. Santovetti,
A. Saputi,
D. Saranin,
A. S.  Sarnatskiy,
G. Sarpis,
M. Sarpis,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
H. Sazak,
L.G. Scantlebury Smead,
A. Scarabotto,
S. Schael,
S. Scherl,
M. Schiller,
H. Schindler,
M. Schmelling,
B. Schmidt,
S. Schmitt,
H. Schmitz,
O. Schneider,
A. Schopper,
N. Schulte,
S. Schulte,
M.H. Schune,
R. Schwemmer,
G. Schwering,
B. Sciascia,
A. Sciuccati,
S. Sellam,
A. Semennikov,
T. Senger,
M. Senghi Soares,
A. Sergi,
N. Serra,
L. Sestini,
A. Seuthe,
Y. Shang,
D.M. Shangase,
M. Shapkin,
R. S.  Sharma,
I. Shchemerov,
L. Shchutska,
T. Shears,
L. Shekhtman,
Z. Shen,
S. Sheng,
V. Shevchenko,
B. Shi,
Q. Shi,
Y. Shimizu,
E. Shmanin,
R. Shorkin,
J.D. Shupperd,
R. Silva Coutinho,
G. Simi,
S. Simone,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
J.C. Smallwood,
E. Smith,
K. Smith,
M. Smith,
A. Snoch,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solomin,
A. Solovev,
I. Solovyev,
R. Song,
Y. Song,
Y. Song,
Y. S.  Song,
F.L. Souza De Almeida,
B. Souza De Paula,
E. Spadaro Norella,
E. Spedicato,
J.G. Speer,
E. Spiridenkov,
P. Spradlin,
V. Sriskaran,
F. Stagni,
M. Stahl,
S. Stahl,
S. Stanislaus,
E.N. Stein,
O. Steinkamp,
O. Stenyakin,
H. Stevens,
D. Strekalina,
Y. Su,
F. Suljik,
J. Sun,
L. Sun,
Y. Sun,
D. S.  Sundfeld Lima,
W. Sutcliffe,
P.N. Swallow,
F. Swystun,
A. Szabelski,
T. Szumlak,
Y. Tan,
M.D. Tat,
A. Terentev,
F. Terzuoli,
F. Teubert,
E. Thomas,
D.J.D. Thompson,
H. Tilquin,
V. Tisserand,
S. T'Jampens,
M. Tobin,
L. Tomassetti,
G. Tonani,
X. Tong,
D. Torres Machado,
L. Toscano,
D.Y. Tou,
C. Trippl,
G. Tuci,
N. Tuning,
L.H. Uecker,
A. Ukleja,
D.J. Unverzagt,
E. Ursov,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
V. Vagnoni,
G. Valenti,
N. Valls Canudas,
H. Van Hecke,
E. van Herwijnen,
C.B. Van Hulse,
R. Van Laak,
M. van Veghel,
G. Vasquez,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V{\'a}zquez Sierra,
S. Vecchi,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Vesterinen,
M. Vieites Diaz,
X. Vilasis-Cardona,
E. Vilella Figueras,
A. Villa,
P. Vincent,
F.C. Volle,
D. vom Bruch,
N. Voropaev,
K. Vos,
G. Vouters,
C. Vrahas,
J. Wagner,
J. Walsh,
E.J. Walton,
G. Wan,
C. Wang,
G. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
N. W.  Wang,
R. Wang,
X. Wang,
X. Wang,
X. W.  Wang,
Y. Wang,
Z. Wang,
Z. Wang,
Z. Wang,
J.A. Ward,
M. Waterlaat,
N.K. Watson,
D. Websdale,
Y. Wei,
J. Wendel,
B.D.C. Westhenry,
D.J. White,
M. Whitehead,
E. Whiter,
A.R. Wiederhold,
D. Wiedner,
G. Wilkinson,
M.K. Wilkinson,
M. Williams,
M.R.J. Williams,
R. Williams,
F.F. Wilson,
W. Wislicki,
M. Witek,
L. Witola,
C.P. Wong,
G. Wormser,
S.A. Wotton,
H. Wu,
J. Wu,
Y. Wu,
K. Wyllie,
S. Xian,
Z. Xiang,
Y. Xie,
A. Xu,
J. Xu,
L. Xu,
L. Xu,
M. Xu,
Z. Xu,
Z. Xu,
Z. Xu,
D. Yang,
K.  Yang,
S. Yang,
X. Yang,
Y. Yang,
Z. Yang,
Z. Yang,
V. Yeroshenko,
H. Yeung,
H. Yin,
C. Y.  Yu,
J. Yu,
X. Yuan,
E. Zaffaroni,
M. Zavertyaev,
M. Zdybal,
C.  Zeng,
M. Zeng,
C. Zhang,
D. Zhang,
J. Zhang,
L. Zhang,
S. Zhang,
S. Zhang,
Y. Zhang,
Y. Z.  Zhang,
Y. Zhao,
A. Zharkova,
A. Zhelezov,
S. Z.  Zheng,
X. Z.  Zheng,
Y. Zheng,
T. Zhou,
X. Zhou,
Y. Zhou,
V. Zhovkovska,
L. Z.  Zhu,
X. Zhu,
X. Zhu,
V. Zhukov,
J. Zhuo,
Q. Zou,
D. Zuliani,
G. Zunica
